Towards Better Fairness-Utility Trade-off: A Comprehensive Measurement-Based Reinforcement Learning Framework

Machine learning is widely used to make decisions with societal impact such as bank loan approving, criminal sentencing, and resume filtering. How to ensure its fairness while maintaining utility is a challenging but crucial issue. Fairness is a complex and context-dependent concept with over 70 different measurement metrics. Since existing regulations are often vague in terms of which metric to use and different organizations may prefer different fairness metrics, it is important to have means of improving fairness comprehensively. Existing mitigation techniques often target at one specific fairness metric and have limitations in improving multiple notions of fairness simultaneously. In this work, we propose CFU (Comprehensive Fairness-Utility), a reinforcement learning-based framework, to efficiently improve the fairness-utility trade-off in machine learning classifiers. A comprehensive measurement that can simultaneously consider multiple fairness notions as well as utility is established, and new metrics are proposed based on an in-depth analysis of the relationship between different fairness metrics. The reward function of CFU is constructed with comprehensive measurement and new metrics. We conduct extensive experiments to evaluate CFU on 6 tasks, 3 machine learning models, and 15 fairness-utility measurements. The results demonstrate that CFU can improve the classifier on multiple fairness metrics without sacrificing its utility. It outperforms all state-of-the-art techniques and has witnessed a 37.5% improvement on average.

==> romeve.tex <==
 
\section{Related Work}\label{chap:relat}
\subsection{Bias Mitigation Techniques} 
Bias mitigation techniques can be classified into three categories, including pre-processing techniques, in-processing techniques and post-processing techniques \cite{cct7}.

Pre-processing techniques are developed based on the assumption that the root cause of unfairness comes from the biased features in training data~\cite{cct9}. Therefore, this family of techniques work on the dataset before training so that models can produce fairer predictions. Preprocessing of data could usually be achieved through the suppression of the sensitive attribute, massaging the dataset by changing class labels, and reweighing or resampling the data to remove discrimination without relabeling instances \cite{cct10}. A representative technique is reweighing \cite{cct11}, which assigns different weights to classes of input according to their degree of being favored \cite{cct6}. Others include modifying feature values \cite{cct12} or feature representations~\cite{cct13,cct14}. Semi-supervised learning framework in pre-processing phase has also been reported \cite{cct15}. However, modifying training data may have unexpected impacts on model fairness \cite{cct16}, and there is huge controversy in the community on whether such action is acceptable.

In-processing techniques modify the ML model to mitigate the bias in predictions. One common technique is adversary training. Usually, adversary training is performed on model level \cite{cct17,cct18,cct19}, but that on individual neuron level has also been developed \cite{cct20}. Like the case in pre-processing techniques, supervised and semi-supervised learning are also applied in some in-processing techniques \cite{cct21,cct22}. Recent studies have proposed special designs for hyperparameters as another possible strategy for improving fairness in ML models \cite{cct23,cct24}. It is worth noting that some pre-processing methods have been integrated in in-processing techniques to form new in-processing ones \cite{cct25,cct26}.

Post-processing techniques modify the prediction results directly for less bias. They remove discrimination by adjusting some predictions of a classifier \cite{AOD}. Multiple post-processing techniques have been developed based on post-hoc disparity \cite{cct28}, Gaussian process \cite{cct29}, group-aware threshold adaptation \cite{cct30}, etc.

In addition to the techniques mentioned above, causality analysis is another way to improve model fairness \cite{cct31,cct32,cct33}. Several strategies like Pareto principle \cite{cct34,cct35} and mutual information \cite{cct36} have been explored in these techniques for better trade-off between fairness and performance.

\subsection{Reinforcement Learning}

Fairness in reinforcement learning was first investigated in 2017 \cite{cct37}. Then the fairness of reinforcement frameworks in real-world applications has been widely studied \cite{cct38,cct39,cct40}. Deep reinforcement learning was also used for fairness testing in ML models \cite{cct41}. However, it should be noted that the studies at that time only cares about the fairness in reinforcement frameworks, rather than improving fairness through RL. It is not until 2021 that RL methods were applied to solve the problems concerning fairness in classification. In this study, Monte Carlo policy gradient method was developed to deal with non-differentiable constraints \cite{cct42}. After that, RL has been used to achieve fairness in recommendation \cite{cct43} and ranking problems \cite{cct44}. Sikdar et al. \cite{getfair} developed a reinforcement framework called \GetFair, which can get competitive accuracy fairness trade-offs across all tested classifier models, datasets, and fairness metrics. However, none of these works have tried to achieve fairness-performance trade-off through the design of reward functions, and the effects of reward functions on fairness-performance trade-off all remain unknown.

In this work, we established a comprehensive measurement for multiple metrics, based on which a new design method for reward function was proposed. Then we proved how the reward function can lead to a better trade-off between fairness and performance, and the metrics suitable for the construction of the reward function were figured out. Compared with other reinforcement frameworks developed for fair classification, our method provides a more intuitive way to achieve better fairness-performance trade-off, and meanwhile has better interpretability.

